Could the recent rebrightening of the GW170817A afterglow be caused by a counter jet?

GRB170817A (also GW170817) became the first binary neutron star (BNS) merger event detected via gravitational waves and electromagnetic signals. Over the next 4 years, various multiband observations have led to re-imagine the various short Gamma Ray Burts (sGRB) and interstellar medium interaction models. While these models successfully explain the observed afterglow until ~900 days, a re-brightening or excess flux was observed in the 1keV X-Ray band after ~1000 days. In this study, we re-evaluate the jet parameters using the new observations (until ~1234 days) with a boosted fireball jet model. We study the observable effects of the counter-jet for GRB170817A, using our new afterglow code, Firefly. Our results show that it is indeed possible for the observed excess to coincide with the emissions from the counter-jet (~800 days). We also computed an empirical scaling law between the jet and counter-jet peak emission timescales and the observer angle. The Firefly code can also track the simulated object through the observers' sky and numerically model the apparent motion. The calculated apparent motion (~2.6c) does not match the observed apparent motion (7.5c to 5.2c). Hence we conclude, the excess flux of GRB170817A may not be associated with the counter jet; however, it is not enough to reject this hypothesis from the traditional counter jet visibility time scales, which predicts > 5000 days. The apparent motion, combined with the multi-band lightcurves, is needed to break degeneracy between geometrical parameters and the microphysical parameters of the afterglow.

==> parameter.tex <==
\setlength{\tabcolsep}{20pt}
\renewcommand{\arraystretch}{1}
\begin{deluxetable*}{|c|c|}
%\tablewidth{0pt}  
\tablecaption{Parameter Range for Fireball Jet} 
\tablehead{ \colhead{Parameter} & \colhead{Double Fireball} }
\startdata
\hline
\hline
$\gamma_B$ & 8.0\\
\hline
$\eta_0$ & 6.5\\
\hline
$\theta_0$ & 7.2\textdegree\\
\hline
$E_{tot}$ & $1.6\times 10^{49} erg$\\
\hline
$E_{iso}$ & $1.98\times 10^{51} erg$\\
\hline
$\theta_{obs}$ & 49.8\textdegree \\
\hline
$n_{ISM}$ & $0.1 cm^{-3}$\\
\hline
p & $2.13$\\
\hline
$\epsilon_e$ & $0.4$\\
\hline
$\epsilon_B$ & $10^{-3}$\\
\enddata
\label{t:parameters}
\tablecomments{\footnotesize{There are eight free parameters in the boosted fireball afterglow model. First two for the jet itself for boosted fireball model ($\gamma_B$, $\eta_0$). The remaining six parameters come from the standard afterglow model. The parameter range for them is chosen according to the physical limits set on them. These are the values for which we find the best agreement between the 3GHz, and 1keV lightcurve. These are the parameters required to correlate the 1keV rebrightening to the counter jet emission for GRB170817. Most notable difference from the previous studies are the values of $n_{ISM}$, and $\theta_{obs}$.}}
\end{deluxetable*}

==> sky_loc.tex <==
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.0}
\begin{deluxetable}{|c | c | c|}
\tablewidth{0pt}  
\tablecaption{Sky Location For GRB170817A with Firefly} 
\tablehead{ \colhead{Distance from merger center} & \colhead{ Time since merge} & \colhead{Apparent velocity}\\
\colhead{$(\times 10^{16} cm)$} & \colhead{(days)} & \colhead{$(cm s^{-1})$}}
\startdata
\hline
\hline
10 & 7.5 & \\
\hline
50 & 29.5 & 2.122 c\\
\hline
75 & 44.5 & 2.354 c\\
\hline
230 & 108.7 & 1.6 c\\
\enddata
\label{t:slyloc}
\tablecomments{There are eight free parameters in the boosted fireball afterglow model. First two for the jet itself for boosted fireball model. The boost of the fireball ($\gamma_B$) constrain the jet opening angle $\theta_0 \in [0.083,0.17] rad$. The remining six parameters come from the stanrdard afterglow model. The parameter range for them is chosen according to the physical limits set on them, via the microphysics governing them.}
\end{deluxetable}
